Analysis of Tree-Algorithms with Multi-Packet Reception

In this paper, we analyze binary-tree algorithms in a setup in which the receiver can perform multi-packet reception (MPR) of up to and including K packets simultaneously. The analysis addresses both traffic-independent performance as well as performance under Poisson arrivals. For the former case, we show that the throughput, when normalized with respect to the assumed linear increase in resources required to achieve K-MPR capability, tends to the same value that holds for the single-reception setup. However, when coupled with Poisson arrivals in the windowed access scheme, the normalized throughput increases with K, and we present evidence that it asymptotically tends to 1. We also provide performance results for the modified tree algorithm with K-MPR in the clipped access scheme. To the best of our knowledge, this is the first paper that provides an analytical treatment and a number of fundamental insights in the performance of tree-algorithms with MPR.

==> WA_exampleAlt.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
{} &   K &     alpha &      beta &    alphaK &     betaK &  lambdaUpper &  lambdaLower &  lambdaDelta &     Delta \\
\midrule
0 &   1 &  2.885383 &  2.885396 &  2.885383 &  2.885396 &     0.429512 &     0.429512 &     1.146218 &  2.668654 \\
1 &   2 &  1.442666 &  1.442720 &  2.885331 &  2.885440 &     0.470676 &     0.470676 &     0.916867 &  1.947979 \\
2 &   4 &  0.721164 &  0.721575 &  2.884657 &  2.886301 &     0.517514 &     0.517514 &     0.799700 &  1.545272 \\
3 &   8 &  0.359075 &  0.362139 &  2.872602 &  2.897112 &     0.567790 &     0.567790 &     0.746098 &  1.314040 \\
4 &  16 &  0.173545 &  0.185899 &  2.776719 &  2.974376 &     0.623877 &     0.623877 &     0.734244 &  1.176904 \\
\bottomrule
\end{tabular}


==> asymptotic.tex <==
\section{Asymptotic Analysis}

In this section, we shed some light on the asymptotic behaviour of conditional \ac{CRI} in case of fair splitting. %, as given by \eqref{eq:BTA_ecri_fair}.
We base the approach on the one the presented in~\cite{MF1985}, done for the standard collision channel. 

%In the previous subsection we have investigated the average resolution length. The $(-1)$ term grants the average an oscillatory behavior with varying number of users. In this subsection we aim to characterize the behavior of these oscillations.
%\CS{Previous work on oscillatory behavior of tree algorithms \cite{MF1985} have demonstrated that the oscillations can be neglected. However, as we will see in Sec.~\ref{sec:eval} that is not the case for MPR trees.}
 
%We investigate an iterative method to derive a different formulation of $L_\nuser$ following the analysis done by Flajolet for $1$-MPR \cite{}.
Rearranging \eqref{eq:step_2_n} for $p = \frac{1}{2}$ yields
\begin{align}
\ecri (x) - 2 \ecri \left( \frac{x}{2}\right) = 1 - 2\sum_{k=0}^{\mpr} \frac{x^k}{k!}  e^{-x}.
\label{eq:step_2_n_asy}
\end{align}
Differentiating \eqref{eq:step_2_n_asy} w.r.t $x$  twice we get,
\begin{align}
\ecri^{''} (x) - \frac{1}{2} \ecri^{''} \left( \frac{x}{2}\right) =  2e^{-x}\left( \frac{x^{K-1}}{(K-1)!} - \frac{x^K}{K!} \right)
\label{eq:diffed_asy}
\end{align}
which is a functional equation in the form
\begin{align}
     f(x) - \frac{1}{2} f\left(\frac{1}{2}x \right) = g(x)\nonumber.
\end{align}
having a unique solution in the form 
 \begin{align}
    f(x) = \sum_{m=0}^\infty \left( \frac{1}{2} \right)^m g \left( \left( \frac{1}{2} \right)^m x \right)
     \nonumber
 \end{align}
as shown in Appendix A of \cite{}.
%For us we have $\gamma=2^{-1}$, $\lambda=0$ and $p=2^{-1}$ and this results in
Thus, the solution of \eqref{eq:step_2_n_asy} is
\begin{align}
\ecri^{''} (x) = 2 \sum_{m=0}^\infty \frac{e^{-\frac{x}{2^m}}}{2^m}\left(\frac{\left(\frac{x}{2^m}\right)^{K-1}}{(K-1)!} - \frac{\left(\frac{x}{2^m}\right)^K}{K!} \right).
\label{eq:diffed_asy_2}
\end{align}

 \eqref{eq:diffed_asy} is a functional equation, i.e.,
 \begin{align}
     f(x) - \gamma f(\lambda + px) = g(x)\nonumber.
 \end{align}
 If $|\gamma|< 1, |p| < 1 $ holds, the equation has a unique solution in the form
 \begin{align}
    f(x) = \sum_{m=0}^\infty \gamma^m g\bigg(\lambda \frac{1-p^m}{1-p} +p^mx\bigg)
     \nonumber
 \end{align}
 as proven in the Appendix A of \cite{}. For us we have $\gamma=2^{-1}$, $\lambda=0$ and $p=2^{-1}$ and this results in
 
 \begin{align}
\ecri^{(2)} (x) = - 2 \sum_{m=0}^\infty 2^{-m}  e^{-x2^{-m}}\left(\frac{(x2^{-m})^{K-1}}{(K-1)!} - \frac{(x2^{-m})^K}{K!}  \right).
\label{eq:diffed_asy_2}
\end{align}


integrating both sides with respect to $x$ twice and using initial conditions $L(0) = 1$ and $L^{(1)}(0) = 0$ \footnote{The initial conditions can be calculated through \eqref{ps_ecri}.}
we get,

\begin{align}
\ecri (x) = 1 - 2\sum_{m=0}^\infty2^me^{-x2^{-m}} \bigg( 1 - \sum_{k=0}^{\mpr} \frac{x^k 2^{-mk}}{k!}  \bigg)
\label{eq:step_3_n_asy}
\end{align}
 that can also be written as,
 
 
\begin{align}
\ecri (x) = 1 - 2\sum_{m=0}^\infty2^me^{-x2^{-m}}  \sum_{k=1}^{\mpr} \frac{x^k 2^{-mk}}{k!}.  
\label{eq:step_3_n_asy}
\end{align}



We know that $L(x)$ has the form

\begin{align}
%\label{ps_ecri_2}
L(x) = \sum^\infty_{n=0} \ecri_\nuser \frac{x^\nuser}{\nuser!}  e^{-x}. \nonumber
\end{align}

We re-formulate \eqref{eq:step_3_n_asy} in order to equate the co-efficients of $\frac{x^\nuser}{\nuser!}  e^{-x}$ which will give us $L_\nuser$. Taking out $e^{-x}$ and expanding the exponential functions with infinite sums we get

\begin{align}
\ecri (x) = e^{-x}e^{x} - e^{-x}\sum_{m=0}^\infty2^{m+1}\sum_{k=1}^{\mpr} \frac{x^k 2^{-mk}}{k!}  {e^{x(1-2^{-m})}}
\nonumber
\end{align}
and

\begin{align}
\label{eq:step_4_n_asy}
\ecri (x) = & \sum_{n=0}^\infty \frac{x^n}{n!}e^{-x}- \nonumber\\ e^{-x}\sum_{m=0}^\infty2^{m+1}\sum_{k=1}^{\mpr} & \frac{x^k 2^{-mk}}{k!}\sum_{n=0}^\infty \frac{x^n (1-2^{-m})^{n}}{n!}
\end{align}

Using the fact that 

\begin{align}
    \sum_{i=0}^n  \frac{(2^{-m})^i (1-2^{-m})^{n-i}}{i!(n -i)!} = 1 \nonumber
\end{align}
We can re-rewrite \eqref{eq:step_4_n_asy} as,


\begin{align}
\ecri (x) = & \sum_{n=0}^\infty \frac{x^n}{n!}e^{-x} -  e^{-x}\sum_{m=0}^\infty2^{m+1}\sum_{n=0}^{\infty} x^n (1 - \frac{(1-2^{-m})^n}{n!})  \nonumber\\  - \sum_{n=K+1}^{\infty} x^n& \sum_{k=K+1}^n \frac{ 2^{-mk}(1-2^{-m})^{n-k}}{k!(n-k)!}
\label{eq:step_5_n_asy}
\end{align}

taking an $n!$ out to equate the coefficients

% \begin{align}
% \ecri (x) = & \sum_{n=0}^\infty \frac{x^n}{n!}e^{-x}- \nonumber\\ e^{-x}\sum_{m=0}^\infty2^{m+1}\sum_{n=0}^{\infty} \frac{x^n}{n!} & \left( n!-\sum_{k=K+1}^n {n \choose k}  2^{-mk}(1-2^{-m})^{n-k}\right)
% \nonumber
% \end{align}

\begin{align}
\ecri (x) = & \sum_{n=0}^\infty \frac{x^n}{n!}e^{-x} -  e^{-x}\sum_{m=0}^\infty2^{m+1}\sum_{n=0}^{\infty} \frac{x^n}{n!} (n! - (1-2^{-m})^n)  \nonumber\\  - \sum_{n=K+1}^{\infty} \frac{x^n}{n!}&\sum_{k=K+1}^n {n \choose k}2^{-mk}(1-2^{-m})^{n-k} \nonumber
%\label{eq:step_5_n_asy}
\end{align}

Grouping the coefficients for $n>K$,

% \begin{align}
% \ecri (x) = \sum_{n=0}^\infty \frac{x^n}{n!}e^{-x}  &\Bigg(1 -  \sum_{m=0}^\infty2^{m+1}  \Bigg( n!-\nonumber\\\sum_{k=K+1}^n  {n \choose k} & 2^{-mk}(1-2^{-m})^{n-k}\Bigg)\Bigg)
% \nonumber
% \end{align}

\begin{align}
\ecri (x) = & \sum_{n=0}^\infty \frac{x^n}{n!}e^{-x}\Bigg( 1 - \sum_{m=0}^\infty2^{m+1}\bigg(n! - (1-2^{-m})^n  \nonumber\\  - &(1-2^{-m})^n\sum_{k=K+1}^n {n \choose k}(1-2^{m})^{-k}\bigg) \Bigg)\nonumber
%\label{eq:step_5_n_asy}
\end{align}


Thus we can re-write the tree length with K-MPR fair BTA as \cite{MF1985},  
% \begin{equation}
%     L_\nuser = 1 - \sum^\infty_{m=0} 2^{m+1} \left[ n! - \sum^n_{k=K+1} {\nuser \choose k}  \frac{(2^m - 1)^{n-k}}{2^{mn} } \right].
% \end{equation}

\begin{align}
 L_\nuser  &=  1 - \sum_{m=0}^\infty2^{m+1}\bigg(n! - (1-2^{-m})^n  \nonumber\\  - &(1-2^{-m})^n\sum_{k=K+1}^n {n \choose k}(1-2^{m})^{-k}\bigg) 
%\label{eq:step_5_n_asy}
\end{align}

This can be re-written as,


\begin{align}
 L_\nuser  &=  1 + \sum_{m=0}^\infty2^{m+1} &(1-2^{-m})^n\sum_{k=1}^K {n \choose k}(1-2^{m})^{-k} 
%\label{eq:step_5_n_asy}
\end{align}

%\mg{after this point is old and to be changed}
Here we assume $\nuser \gg 1$ and re-write this as,

\begin{align}
 L_\nuser  & \approx 1 + \sum_{m=0}^\infty2^{m+1} &(1-2^{-m})^n\sum_{k=1}^K \frac{(1-2^{m})^{-k}}{k!} 
%\label{eq:step_5_n_asy}
\end{align}
 \begin{equation}
     L_\nuser \approx 1 + 2\sum^\infty_{k=0} 2^k  \left( \frac{1}{2^k - 1}\right)^\nuser \left[ 1 - \sum^\mpr_{j=0} \frac{1}{j!}\left( \frac{\nuser}{2^k - 1}\right)^j  \right].
 \end{equation} 
%To achieve this we start with a change of variable as $V =\left( \frac{\nuser}{2^k - 1}\right)$.

As this form is not so easy to analyze we apply a Mellin transform to the equation. Moreover taking the Mellin transform $L_\nuser$ and formulating the inverse transform we get,

\begin{equation}
    L_\nuser  \approx 1 - \frac{2}{2\pi i} \int_{-3/2 -i\infty}^{-3/2+i\infty} \frac{\sum^\mpr_{j=0}\frac{s^j}{j!}}{1 - 2^{s+1}} \Gamma(s) \nuser^{-s} ds . 
\label{eq:mellin_tree}
\end{equation}

Using residual theorem we can complete the inverse Mellin transform in \eqref{eq:mellin_tree}. The result expresses the oscillations of the K-MPR tree algorithm. The pole at $ \frac{2\pi i k}{\text{ln}2} - 1$, stemming from the denominator had to be taken in to account and this results in,

\begin{equation}
    L_\nuser \approx 1 -\frac{2\nuser}{\text{ln}2}
    \sum_{k\neq0} \Gamma\left(\frac{2\pi i k}{\text{ln}2} - 1\right)\sum^\mpr_{j=0} \frac{(2\pi i k-1)^j}{j!}\nuser^{\frac{-2\pi i k}{\text{ln}2}}.
\end{equation}

The Gamma function in the sum over $k$ depicts the oscillatory behavior, i.e., the frequency of the oscillations. We see that this parameter does not depend on $\mpr$. So the frequency of the oscillations are the same with respect to $\mpr$. The sum on the right taken up to $\mpr$ is setting the magnitude of the oscillations. Thus, varying $\mpr$ will increase the variance of the throughput. This is an interesting result that we will discuss in Sec.~\ref{sec:eval}. % This holds with our observations as the oscillations grow with increasing MPR. 


==> windowed_lambda.tex <==
1 0.42951
2 0.47068
4 0.51751
8 0.56779
10 0.5850039
16 0.62388
20 0.6435351
30 0.6802734
40 0.7063453
50 0.7262098
100 0.7835304
200 0.8324254
500 0.8832808
1000 0.9123721
